Second-Order Functions and Theorems in ACL2

SOFT ('Second-Order Functions and Theorems') is a tool to mimic second-order functions and theorems in the first-order logic of ACL2. Second-order functions are mimicked by first-order functions that reference explicitly designated uninterpreted functions that mimic function variables. First-order theorems over these second-order functions mimic second-order theorems universally quantified over function variables. Instances of second-order functions and theorems are systematically generated by replacing function variables with functions. SOFT can be used to carry out program refinement inside ACL2, by constructing a sequence of increasingly stronger second-order predicates over one or more target functions: the sequence starts with a predicate that specifies requirements for the target functions, and ends with a predicate that provides executable definitions for the target functions.

==> eptcsdata.tex <==
\providecommand{\firstpage}{17}
\providecommand{\publicationstatus}{M. Kaufmann and D. Rager (Eds.): ACL2 Workshop 2015 (ACL2 2015).\\
EPTCS 192, 2015, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.192.3}{10.4204/EPTCS.192.3}}
\pdfoutput=1

